The Sampling-Gaussian for stereo matching

The soft-argmax operation is widely adopted in neural network-based stereo matching methods to enable differentiable regression of disparity. However, network trained with soft-argmax is prone to being multimodal due to absence of explicit constraint to the shape of the probability distribution. Previous methods leverages Laplacian distribution and cross-entropy for training but failed to effectively improve the accuracy and even compromises the efficiency of the network. In this paper, we conduct a detailed analysis of the previous distribution-based methods and propose a novel supervision method for stereo matching, Sampling-Gaussian. We sample from the Gaussian distribution for supervision. Moreover, we interpret the training as minimizing the distance in vector space and propose a combined loss of L1 loss and cosine similarity loss. Additionally, we leveraged bilinear interpolation to upsample the cost volume. Our method can be directly applied to any soft-argmax-based stereo matching method without a reduction in efficiency. We have conducted comprehensive experiments to demonstrate the superior performance of our Sampling-Gaussian. The experimental results prove that we have achieved better accuracy on five baseline methods and two datasets. Our method is easy to implement, and the code is available online.

==> src/chap2_0.tex <==



In the fields of cryptography and privacy protection, Laplace and Gaussian distribution are leveraged for noise add to the real numbers to protect privacy. The discrete Gaussian distribution \cite{NIPS2020_DiscreteGaussian} 
% Recently, the discrete Gaussian distribution \cite{NIPS2020_DiscreteGaussian} 
\begin{definition}[Discrete Gaussian]
\textit{
   let $\mu,\sigma \in \mathbb{R}$ with $\sigma>0$. The discrete Gaussian distribution is denoted $\mathcal{N}_{Z}(\mu,\sigma^{2})$. The probability distribution is defined by, $ \forall x \in \mathbb{Z},$
   }
\begin{equation}
   \underset{X\leftarrow \mathcal{N}_{\mathbb{Z}}(\mu,\sigma^{2})}{\mathbb{P}}[X=x]=\frac{e^{-(x-\mu)/2\sigma^{2}} }{\sum_{y\in S}e^{-(y-\mu)/2\sigma^{2}}}.
   \label{DiscreteGaussian}
\end{equation}
\end{definition}
The summation in denominator ensures that the sum of the $\mathbb{P}$ equals $1$.
The discrete Gaussian is supported on a broader domain of definition. 
On the other hand, our sampling-Gaussian is defined only on $S$.

% Then we conduct an empirical analyses of the reason why previous method have failed. Based on the two analyses, we introduce our 
Simultaneously, we also perform an in-depth exploration of the reasons why previous methods for constructing supervision signals fail to effectively enhance accuracy. Building on the above analysis, we introduce our proposed sampling-Gaussian method. In Chapter 3, we theoretically expound the reasons for the effectiveness of supervision signals. Additionally, we redesign the disparity interval selection method for upsampling and cost volume. Furthermore, we devise a combined loss function for training purposes. Moreover, the 



To address those problems, we propose a novel supervising signal construction and training method for stereo matching called \textit{Sampling-Gaussian}. As shown in Fig. \ref{fig1}, our method achieves notable improvement over all the baselines. Additionally, our method does not rely on Top-k or any other post-processing. Therefore, our method can be directly applied to any stereo matching algorithms based on \textit{soft-argmax} without decrease in efficiency.

    

% will not lead to a decrease in efficiency and can be directly transplanted to all current depth estimation algorithms based on soft-argmax.









% \cite{Chen_2019_ICCV, Xu_2024_CVPR}
% 上述提到的

% In this paper, we thoroughly investigate the cause of ambiguous matching by analyzing the training process. We have identified that \textit{soft-argmax} introduces biased gradients during backpropagation, affecting the network's performance.



% the unstable gradients caused by \textit{soft-argmax} during backpropagation.
% \textit{soft-argmax} for disparity regression during training.
% inacurate
% the \textit{soft-argmax} for disparity regression.
% gradients of \textit{soft-argmax} during backpropagation and discovered the unstable gradients would lead to the shift of distribution. 
% Therefore, we omitted \textit{soft-argmax} during training and leverage Gaussian distribution as supervision signal to provide explicit constraint for the shape of the distribution after \textit{softmax}.
% As shown in Fig. \ref{fig1}, the distribution trained with \textit{soft-argmax} exhibits a steep unimodal distribution, making it sensitive to minor changes in probability. On the other hand, the distribution trained with sampling-Gaussian exhibits a moderate probability and is consistent with the probability of a Gaussian distribution.
% Our proposed \textbf{sampling-Gaussian} can be applied to any \textit{soft-argmax}-based method directly without alteration to the network.
% The mathematical proofs are provided in Section $\ref{section3}\& \ref{section4}$. 

Therefore, we omitted \textit{soft-argmax} during training and leveraged the Gaussian distribution as a supervision signal to provide explicit constraints for the shape of the distribution after \textit{softmax}. As shown in Fig. \ref{fig1}, the distribution trained with \textit{soft-argmax} exhibits a steep, unimodal distribution, making it sensitive to minor changes in probability. On the other hand, the distribution trained with sampling-Gaussian exhibits a moderate probability and is consistent with the probability of a Gaussian distribution. Our proposed \textbf{sampling-Gaussian} can be applied directly to any \textit{soft-argmax}-based method without altering the network. Mathematical proofs are provided in Sections $\ref{section3}$ and $\ref{section4}$. An illustration of the workflow is provided in appendix \ref{workflow}.

% On the other hand, the distribution trained with \textit{soft-argmax} shows a steep unimodal.


% Stereo matching is a fundamental task in computer vision, and deep neural network-based methods have achieved significant success in this field. The GC-net \cite{GC-net} was the first to leverage \textit{soft-argmax} for the regression of disparity, and achieving superior results compared to others. Based on this baseline, numerous new studies \cite{chang_pyramid_2018,pan_multi-stage_2020,wang2021pvstereo,ACVnet,shen2023digging} have introduced various novel models and modules to improve accuracy. Nevertheless, soft-argmax remains a key component of those methods due to its simplicity and efficiency.




% **** introduce the soft-argmax in detection



% However, during our study of the stereo matching, we discovered the probability map follows a certain pattern and very similar to a Gaussian distribution.

% \textit{soft-argmax} is equivalent to calculates the expectation of the distribution. Then the penalty on the expectation is same as penalty to the mean of the distribution. Therefore, it lacks explicit constraint to the shape of distribution. However, during our study, this is not the case for stereo matching.

% the shape of the distribution lacks a explicit constraint
% noticed the \textit{soft-argmax} lacks of explicit constraint to variances of the probability map and proposed to construct a variant-aware loss.



% As for the area of stereo matching,
% In the field of stereo matching, the strengths and weaknesses of \textit{soft-argmax} are also extensively discussed. 

% 因此一些方法把不准确估计的原因归结于多模问题。


% 在第三章，我们对网络的训练趋势进行了分析。并且发现，真正影响网络表现的是在训练后期，分配的微调阶段。而这些问题都可以通过我们提出的采样高斯来解决。


% Our proposed \textbf{sampling-Gaussian} 
% The contribution of our work includes three folds,
% In section \ref{section3}, 
In Section \ref{section3}, we start by describing the observed phenomena during our research. We then analyze and identify the reason for inaccurate results: the biased gradients caused by \textit{soft-argmax}. In Section \ref{section4}, we propose \textbf{sampling-Gaussian}, a sampling method based on the Gaussian distribution. We theoretically analyze the properties of sampling-Gaussian and conduct comprehensive experiments to demonstrate its superiority over other methods. Our method effectively improves the network's accuracy.

In summary, the contributions of this work are threefold:

\input{src/figandtable/analyze.tex}

% With the deepening research on disparity estimation, deeper structures and complex modules have indeed achieved more accurate results. 
% This indirectly confirms Kendall's assertion\cite{GC-net}, but the issue of multimodal still exists for lighter models. 
% Therefore, the fundamentaemize}



% With the deepeningl problemize}



% With the deepeningem of \emize}



% With the deepeningtextit{soft-argmax} remains unresolved.




% GC-net\cite{GC-net}
%  have focused on the multimodal distribution of \textit{soft-argmax} in stereo matching and dedicated to mitigate the impact it brings. However, the 


% And stereo matching, there are a main difference, first the index number of \textit{soft-argmax} is relatively large, 192. We observe that the large index could lead to unstable gradients. In Section 3, we give detailed analysis of this observation.

% And 
% Second, the 




% The GC-net \cite{GC-net} has proposed an end-to-end CNN to aggregate the disparity cost volume. And they leverage the soft-argmax for the regression of disparity
% Their baseline has been commonly 




% But how to improve the accuracy of 
% Deep conventional neural network-based methods 
% Deep conventional neural network-based methods have proven to be effective in the field of stereo matching. 


% Common approaches can be divided into two categories: matching-based and aggregation-based .

% The matching-based method \cite{Mayer2016CVPR} train the network by end-to-end to regression the network 

% The aggregation-based methods\cite{GC-net,chang_pyramid_2018,pan_multi-stage_2020,ACVnet,} train the end-to-end CNN to aggregate the cost volume and regression the disparity. The GC-net \cite{GC-net} first leverages the soft-argmax for the regression of disparity. This method has been commonly adopted in the 









==> src/chap2_pre_copy.tex <==

\section{Related Works}
% \label[type]{section2}
\subsection{\textit{Softmax}, \textit{soft-argmax} and disparity regression}
The \textit{argmax} retrieves the index of the highest probability. And the operation \textit{soft-argmax}\cite{goodfellow2016deep} is a differentiable approximation of \textit{argmax}. Disparity regression \cite{GC-net} leverages \textit{soft-argmax} to calculates the disparity.
\begin{definition}[Disparity Regression]
   \label{disparityregression}
\textit{
   Define a neural network $f: \mathbb{R}^{3} \rightarrow \mathbb{R}^{d_{max}}$ by $z=f(x)$. 
   Set $S = \{i| i\in \mathbb{Z}, 0\leqslant x <d_{max}\}$.
   The disparity regression supported on $S$ is defined by $\forall i \in S$, 
}
% \begin{equation}
%    d =  \sum_{i} i*softmax(z_{i}) =\sum_{i} i*\frac{e^{z_{i}}}{\sum e^{z_{i}}}.
% \label{softargmax}
% \end{equation}
\end{definition}
The $d$ denotes the output disparity, and hypeparameter $d_{max}$ is set to $192$ \cite{chang_pyramid_2018}. 
% The $f(\cdot)$ is stacked conventional layers. And disparity regression is the last layer of the network.
The network is trained end-to-end with $smoothl1$ loss.
\begin{equation}
smoothl1(d,\hat{d}) = \left\{\begin{matrix}
   0.5(d-\hat{d})^{2},& if |d-\hat{d}|<1\\
   |d-\hat{d}|-0.5,& otherwise
   \end{matrix}\right.,
\end{equation}
$\hat{d}$ denotes the ground truth.


\subsection{Discrete Gaussian Distribution}
In the fields of cryptography and privacy protection, Laplace and Gaussian distribution are levreaed for noise add to the real numbers to protect privacy. The discrete Gaussian distribution \cite{NIPS2020_DiscreteGaussian} 
% Recently, the discrete Gaussian distribution \cite{NIPS2020_DiscreteGaussian} 
\begin{definition}[Discrete Gaussian]
\textit{
   let $\mu,\sigma \in \mathbb{R}$ with $\sigma>0$. The discrete Gaussian distribution is denoted $\mathcal{N}_{Z}(\mu,\sigma^{2})$. The probability distribution is defined by, $ \forall x \in \mathbb{Z},$
   }
\begin{equation}
   \underset{X\leftarrow \mathcal{N}_{\mathbb{Z}}(\mu,\sigma^{2})}{\mathbb{P}}[X=x]=\frac{e^{-(x-\mu)/2\sigma^{2}} }{\sum_{y\in S}e^{-(y-\mu)/2\sigma^{2}}}.
   \label{DiscreteGaussian}
\end{equation}
\end{definition}
The summation in denominator ensures that the sum of the $\mathbb{P}$ equals $1$.
The discrete Gaussian is supported on a broader domain of definition. 
On the other hand, our sampling-Gaussian is defined only on $S$.
% Compared to our sampling-Gaussian, 
% Compared to disparity regression, the discrete Gaussian provides a broader domain of definition.
% It's designed to ensure that the sum of the discrete Gaussian equals $1$.
% They addressed a crucial issue by utilizing fractional form, namely, that the sum of the discrete Gaussian is not strictly equal to $1$.

==> src/chap3_analysis.tex <==

\subsection{Analysis}
% Before we started
% \textbf{Lemma 2.1}. \textit{
%     The distribution
% }

% Since we aim to analyze the changes in the model during training, it is essential to analyze the gradients during backpropagation.
% \textbf{Analysis 1}: \textit{The network collapse during training}
% During the experiments, we noticed a repeated issue where the model experiences temporary collapses during the early stages of training, as shown in the fig \ref{fig_for_illustration} (a). 
% Based on the three observations, we deduce that the problem arises during the training process.
The three observations are all related to the training process; therefore, we started by analyzing gradients generated by \textit{softmax} during the backpropagation process.
% , we present a similarity matrix by computes the difference between different index
% In fig. \ref{fig_for_illustration} (c), we 
% 我们对比了在训练初期e所接受的概率。其中相似矩阵所对比的是梯度值的大小,侧边的bar所展示的是归一化后的值。坐标轴中的值，是 abs(i-argmax)。可以看到整个梯度是无序的，而越远离中心值的位置所得到的梯度越大。这一观察与我们前面的假设一致。但是这一个原因也是因为这时的概率的分布是无序的。


The $e^{z_{i}}$ is an element of \textit{softmax}'s output, $z_{i}$ denotes the previous layer, which is the input of \textit{softmax}. The partial derivative of \textit{$e^{z_{i}}$} is defined as Equ. \ref{preliminary}, and the detail of equation is provided in the Appendix \ref{a1}.
The variable $i$ denotes the corresponding index, and $d$ denotes the result of Equation \ref{softargmax}.
As listed following, the derivative of $e^{z_{i}}$ is the product of, the partial derivative $\frac{\partial L}{\partial d}$, the probability of $z_{i}$, and the distance of $i$ to $d$. Specifically, only the last two items have correlation with index $i$. 
\begin{equation}
\begin{aligned}
\frac{\partial L}{\partial e^{z_{i}}}
&=\frac{\partial L}{\partial d}\frac{\partial d}{\partial e^{z_{i}}}\\
&=
\frac{\partial L}{\partial d}(i\frac{e^{z_{i}}}{\sum e^{*}}(1-\frac{e^{z_{i}}}{\sum e^{*}})\\
&+\sum_{j\neq i}j(-\frac{ e^{z_{j}}}{\sum e^{*}}*\frac{e^{z_{i}}}{\sum e^{*}}))\\
&=\frac{\partial L}{\partial d}(\frac{ e^{z_{i}}}{\sum e^{*}}({ i}-d)).
\end{aligned}
\label{preliminary}
\end{equation}
% 根据我们的观察1， 可以得知，距离中心越远的 index对于最后的结果影响越小，根据equ，他们的梯度总是会被乘以一个更大的系数。但是这个系数同时又受到 概率项的影响，因此这个概率项是最终梯度的关键。
% The probability of $z_{i}$ varies from $0.1$ to $1^{-10}$.
% 根据我们的观察1， 可以得知
The $i-d$ ranges from $0$ to $192$, and the probability $\frac{ e^{z_{i}}}{\sum e^{*}}$ varies from $10^{-1}$ to $10^{-10}$. 
We can infer that indices farther from $d$ would consistently receive a larger weight from $i-d$, but the probability has the potential to balance out the impact due to the significant scale difference. Therefore, we conducted analyses at two stages of the network: the early and late stages of training.
% when the neural network is not stable, and the late stage when the network has converged.
% , considering most distributions are unimodal. 
% However, at the early stage of training, the neural network is not stable, and the distributions vary in shape.
% \input{src/figandtable/mygauss_fig.tex}
\input{src/figandtable/flow.tex}

\textbf{At the initial stage of training}, the neural network experiences a period of instability, and the varied shape of $\frac{e^{z_{i}}}{\sum e^{}}$ would result in an unstable gradient.
% and the inferred $\frac{e^{z_{i}}}{\sum e^{}}$ does not follow a unimodal distribution. 
% and the varied shape of $\frac{e^{z_{i}}}{\sum e^{}}$ would resulting a unstable gradient
% To validate our theory, we conducted a comparison of the gradients obtained by nodes $z^{*}$ before the \textit{softmax} operation. As shown in Fig. \ref{fig_for_illustration} (c), the similarity matrix contrasts the gradient magnitudes, with sidebars illustrating normalized values, brighter colors correspond to larger magnitudes. Axis ticks represent $|i-d|$, signifying the distance of indices from $d$. The similarity matrix has corroborated our conjecture that the gradient for each index is proportional to $|i-d|$. Consequently, these excessively large gradients destabilize the training process, resulting in \textbf{Observation} 2.
To validate our theory, we compared the gradients obtained by nodes $z^{*}$. As shown in Fig. \ref{fig_for_illustration} (c), the similarity matrix contrasts the gradient magnitudes, with sidebars illustrating normalized values; brighter colors correspond to larger magnitudes. Axis ticks represent the range of $|i-d|$, signifying the distance of indices from $d$. The similarity matrix has corroborated our conjecture that the gradient for each index is proportional to $|i-d|$. Consequently, these excessively large gradients destabilize the training process, resulting in \textbf{Observation 2}.


% with larger larger gradients obtained at positions farther from the center value. This observation supports our earlier assumption.
% reveals that the overall gradient is disordered, 
% with larger gradients obtained at positions farther from the center value. This observation supports


% It can be observed that the entire gradient is disordered, with larger gradients obtained at positions farther from the center value. This observation aligns with our earlier assumption. However, this is also because the distribution of probabilities at this stage is disordered
% have a smaller impact on the final result. 
% According to the equation, their gradients are consistently multiplied by a larger coefficient. However, this coefficient is also influenced by the probability term, underscoring the significance of this probability term in determining the final gradient.
% On the other hand the probability varies from $1^{-1}$ to $1^{-10}$. Therefore, the impact of $i-d$ varies.
% We analyzed the gradients during different stages of model training and observed that the impact of $i-d$ is particularly severe in the early stages of training. 
% We compared the gradients that each element $e^{z^{*}}$ of \textit{softmax} received in the early stages of training,  





% 我们还对比了训练后期的概率，可以看到所获得的梯度基本稳定下来了，而其中主要的原因是概率分布基本稳定了，基本符合unimodal了。而在中心以外的位置的概率很低，而因为概率与i-d之间的量级差距很大，所以即使乘上i-d, 它的梯度也不会有太大变化。但是在中心附近的概率基本很接近，因此及时乘上2,3倍数，也会导致梯度变得特别大。

% As training continues, the problem tends to alleviate due to the significant difference in magnitudes between the first two terms.


% As training progresses, the model gradually stabilizes, and the distribution of $\frac{e^{z_{i}}}{\sum e^{}}$ demonstrates unimodality. Consequently, the impact of $i-d$ gradually diminishes, given that the distant index typically possesses lower probabilities.
% We also compared the probabilities in the later stages of training, and it can be observed that the obtained gradients have stabilized. The main reason for this is that the probability distribution has become stable, essentially conforming to a unimodal distribution. The probabilities at positions outside the center are very low, and due to the significant magnitude difference between probability and (i-d), even if multiplied by (i-d), the gradient will not change much. However, the probabilities near the center are quite close, so even multiplying by a factor of 2 or 3 can lead to significantly larger gradients.

\textbf{As training progresses}, the neural network gradually stabilizes, and the distribution of $\frac{e^{z_{i}}}{\sum e^{}}$ exhibits order and unimodality. Consequently, the influence of $i-d$ on distant indices gradually balances out by probabilities, as distant indices typically bear very small probabilities.

However, the probabilities near the peak of the unimodal distribution are very close; therefore, even multiplication by a factor of $2$ or $3$ can lead to significantly larger gradients. As illustrated in Fig. \ref{fig_for_illustration} (d), we compared the received gradients in the later stages, and the matrix has also substantiated our conjecture. Regarding \textbf{Observation 3}, in the final fine-tuning stage, it relies on changing the distribution to precisely fit the target value. However, as the surrounding distribution always receives a relatively large gradient, the model would ultimately oscillate near the optimum without reaching it.

% so even a multiplication by a factor of 2 or 3 can result in significantly larger gradients.
% However, the probabilities near the center are closely distributed, so even a multiplication by a factor of 2 or 3 can result in significantly larger gradients.


% In addition, we conducted a comparison of probabilities during the later stages of training, revealing that the acquired gradients have stabilized. This stabilization can be attributed to the probability distribution becoming consistent and conforming to a unimodal pattern. The probabilities at positions outside the center are very low, and due to the substantial magnitude difference between the probability and $(i-d)$, even when multiplied by $(i-d)$, the gradient undergoes minimal change. 

% 而对于前面提到的观察3。在最后的微调阶段，就是依靠改变分布的比例来精确拟合目标值，但是如果周边分布总是会得到一个较大的梯度，那么最后只会导致模型总是在最优解的附近震荡，而无法到达最优点。





% 这样的训练方式从根本上有问题，因此，我们决定提出一个直接的训练方式，以交给

% The distance of $i$ to $d$ determines that when $i$ is far from $d$, $z_{i}$ will receive a larger gradient.
% \textbf{Proposition 3.1}. \textit{
% Given $(i-d) \in [0,d_{max})$. $\frac{\partial L}{\partial e^{z_{i}}} \propto (i-d)$. \textit{$e^{z_{i}}$} with index away from $d$, would receive greater gradients. Let $\Delta > 0$,$|\frac{ e^{z_{i}}}{\sum e^{*}}| = \Delta$. The $\Delta$ decides the gradients
% }

% Is the training, the network 
% Therefore, we deduced that the cause of collapse is the exceptionally large gradients.
% 我们归纳不稳定的训练的原因是特大的梯度。也因此引出我们接下来的分析，具体量化这些梯度。
% \textit{\textbf{Analysis 2}: The unstable gradient at the early stage}

% \subsection{The gradients}
% 我们对训练中不同阶段的模型训练时的梯度进行了分析，然后发现在训练初期，这个问题会特别的严重，而到后期时，这个问题会因为前两项的量级差距太大而减轻，

% The $i-d$ ranges from 0 to 192. on the other hand the probability ranges from 0 to 1. 
% The $i-d$ ranges from 0 to 192.
% Therefore,





% 训练初期的梯度本来就不稳定，前面的系数放大了这种不稳定。因此我们把训练初期的梯度进行了可视化，
% As fig \ref{fig_for_illustration} (b) shown,


% \textit{\textbf{Analysis 3} The probability changes during the }


% \textit{\textbf{Analysis 4} The gradient at the later stage}



% As the Equ. \ref{preliminary} shows


% % 插入一张图or其他方式，说明在不稳定的时候，
% \textbf{the }



% \textbf{the learning trajectories}
% the network trained with 



==> src/figandtable/abal_gaussiansigma_image.tex <==
\begin{figure}[ht]
    \centering
    \subfigure[Input]{
        \includegraphics[width=0.30\linewidth]{fig/comp_sigma/col.png}
    }
    \subfigure[$\sigma=1.0$]{
        \includegraphics[width=0.30\linewidth]{fig/comp_sigma/d07.png}
    }
    \subfigure[$\sigma=1.3$]{
        \includegraphics[width=0.30\linewidth]{fig/comp_sigma/d13.png}
    }
    \caption{The estimated disparities by the network trained with various $\sigma$ are presented in gray instead of pseudo-color to better illustrate the blurred contour.}
    \label{comp_sigma}
\end{figure}


==> src/figandtable/abal_klvsl1.tex <==
\begin{table}[ht]
\centering
\caption{Comparisons of KLdiv and smoothl1}
\begin{tabular}{lcc}
\toprule
    & KLdiv    & \textbf{smoothl1}\\\midrule
    MSNet2D   &$   1.366 $&$  \textbf{0.897}     $\\
PSMnet &$  0.719   $&$  \textbf{0.625}   $\\
\bottomrule
\end{tabular}
\label{Comparisons of KLdiv and smoothl1}
\end{table}

==> src/figandtable/abal_samplingVSdiscrete.tex <==
\begin{table}[h]
\centering
\caption{Comparisons(EPE) of SG and DG. }
\begin{tabular}{lccc}
\toprule
& \textit{soft-argmax} & $DG$ & \textit{\textbf{SG}} \\\midrule
MSNet2D  &$     0.932      $&$   1.295   $&$ 0.897 $\\
PSMnet &$     0.748      $&$   0.704     $&$   0.625 $\\\bottomrule
\end{tabular} 
\label{Comparisons of SG and DG.}
\end{table}

==> src/figandtable/abal_samplingVSdiscrete_Fig.tex <==
\begin{figure}[ht]
\centering
% \includegraphics[width=0.49\linewidth]{fig/cumu4.png}
\includegraphics[width=0.95\linewidth]{fig/cumu5.png}

\caption{The left plot is the comparison between Discrete-Gaussian and proposed sampling-Gaussian. The right plot is the comparison between training with KL divergence and smoothl1.}
\label{trainingcurve}
\end{figure}

==> src/figandtable/analyze.tex <==
\begin{figure*}[!htbp]
    \centering
    \subfigure[]{\includegraphics[width=0.24\linewidth, height=0.2\linewidth]{fig/lines.png}}
    \subfigure[]{\includegraphics[width=0.24\linewidth, height=0.2\linewidth]{fig/246.png}}
    \subfigure[]{\includegraphics[width=0.24\linewidth]{fig/difference_begin.png}}
    \subfigure[]{\includegraphics[width=0.24\linewidth]{fig/difference_end.png}}
    \caption{
    Illustrations of the observations and analysis:
    (a) The lines indicate four different training trajectories with random initialization, and the collapses of the network are highlighted.
    (b) The plot illustrates the evolution of the distribution at three distinct epochs. The triangle represents each index's respective probability at the specified epoch.
    (c) A similarity matrix illustrating the magnitude of gradients at the initial stage of training.
    (d) A similarity matrix illustrating the magnitude of gradients at the late stage of training.
    }
    \label{fig_for_illustration}
 \end{figure*}

==> src/figandtable/dg_ana.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.8\linewidth]{fig/dg_ana.png}
\caption{The changing of probability. The $1-\sum p$ represents the difference between the probability sum and $1$.}
\label{da_ana}
\end{figure}

==> src/figandtable/flow.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/flow.jpg}    
    \caption{workflow}
\end{figure}

==> src/figandtable/q_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lcccccc}
            & all  &       &       & noc   &       &       \\
            & d1bg & d1fg  & d1all &  1.71 &  4.31 &  2.14 \\
msnet2d     & 2.49 &  4.53 &  2.83 &  2.29 &  3.81 &  2.54 \\
sg-msnet2d  & 1.94 &  4.07 &  2.29 &  1.78 &  3.63 &  2.08 \\
psmnet      & 1.86 &  4.62 &  2.32 &  1.71 &  4.31 &  2.14 \\
sg-psmnet   & 1.77 &  3.13 &  2.00 &  1.65 &  2.97 &  1.87 \\
gwcnet-g    & 1.74 &  3.93 &  2.11 &  1.61 &  3.49 &  1.92 \\
sg-gwcnet-g & 1.73 &  3.88 &  2.09 &  1.59 &  3.55 &  1.92 \\
msn3d       & 1.75 &  3.87 &  2.10 &  1.61 &  3.50 &  1.92 \\
sg-msn3d    & 1.61 &  3.81 &  1.98 &  1.48 &  3.55 &  1.82 \\
            &      &       &       &       &       &       \\
            &      &       &       &       &       &       \\
            &      &       &       &       &       &       \\
igev        & 1.38 &  2.67 &  1.59 &  1.27 &  2.62 &  1.49 \\
sg-igev     & 1.40 &  2.50 &  1.58 &  1.30 &  2.48 &  1.50
\end{tabular}
\end{table}
